A Study of Editor Features in a Creative Coding Classroom

Creative coding is a rapidly expanding domain for both artistic expression and computational education. Numerous libraries and IDEs support creative coding, however there has been little consideration of how the environments themselves might be designed to serve these twin goals. To investigate this gap, we implemented and used an experimental editor to teach a sequence of college and high-school creative coding courses. In the first year, we conducted a log analysis of student work (n=39) and surveys regarding prospective features (n=25). These guided our implementation of common enhancements (e.g. color pickers) as well as uncommon ones (e.g. bidirectional shape editing). In the second year, we studied the effects of these features through logging (n=39+) and survey (n=23) studies. Reflecting on the results, we identify opportunities to improve creativity- and novice-focused IDEs and highlight tensions in their design -- as in tools that augment artistry or efficiency but may be perceived as hindering learning.

==> commands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\toolName}[1]{#1}
\newcommand{\sns}{\toolName{Sketch-n-Sketch}}

\newcommand{\osf}{\url{https://osf.io/cture/}}

\newcommand{\etal}
{et al.}
%% {et al.\@ }
\newcommand{\etals}
{et al.'s}
%% {et al.\@'s }  

\newcommand{\ie}{{i.e.}}
\newcommand{\eg}{{e.g.}}
\newcommand{\etc}{{etc.}}
\newcommand{\cf}{{cf.}}


% \newcommand{\hideComments}{HIDE EM} % comment out to allow comments
\ifx\hideComments\undefined
  %% Do this if it is undefined
  \newcommand\rc[1]{{\color{blue}[RC: #1]}}
  \newcommand\am[1]{{\color{red}[AM: #1]}}
  \newcommand{\todo}[1]{\textcolor{magenta}{\textsf{{#1}}}}
\else
  %% Do this if it is defined
  \newcommand\rc[1]{{}}
  \newcommand\am[1]{{}}
  \newcommand{\todo}{{}}
\fi

\newcommand{\authorVersion}{HIDE EM} % comment out to allow comments
\ifx\authorVersion\undefined
  %% Do this if it is undefined
  \newcommand\spaceit[0]{\vspace{-0.2in}}
  % \newcommand\spaceit[1]{\vspace{#1}}
\else
  %% Do this if it is defined
  \newcommand\spaceit[0]{{}}
  % \newcommand\spaceit[1]{}
\fi


\newcommand{\theAppendix}{the appendix}

% Use these instead of \autoref ?
\newcommand{\secref}[1]{\hyperref[#1]{Sec.~\ref*{#1}}}
\newcommand{\appendixref}[1]{\hyperref[#1]{Appendix.~\ref*{#1}}}
\newcommand{\figref}[1]{\hyperref[#1]{Fig.~\ref*{#1}}}
\newcommand{\eqnref}[1]{\hyperref[#1]{Eqn.~\ref*{#1}}}
\newcommand{\tabref}[1]{\hyperref[#1]{Table ~\ref*{#1}}}

% https://tex.stackexchange.com/questions/74212/how-can-i-change-the-whitespace-above-and-below-center
\newenvironment{mycenter}[1][\topsep]
{\setlength{\topsep}{#1}\par\kern\topsep\centering}% \begin{mycenter}[<len>]
{\par\kern\topsep}

\newcommand{\footnoteWithIndent}[1]
{\footnote{\mbox{}\hspace{0.01in}{#1}}}
%% {\footnote{#1}}


\newcommand{\imm}{\emph{su21}}
\newcommand{\csp}{\rc{REMOVE \emph{su21-lite}}}
\newcommand{\spq}{\emph{sp21}}
\newcommand{\wiq}{\emph{wi22}}
\newcommand{\sumtwo}{\emph{su22}}

%% TODO try controlling the space around equals like this elsewhere too
\newcommand{\nEquals}[1]
%% {\ensuremath{(n=#1)}}
{($n$=#1)}
% {\mbox{($n$\hspace{0.03in}$=$\hspace{0.03in}#1)}}
\newcommand{\numYearOneLog}{39}
\newcommand{\numYearOneSurvey}{25}
\newcommand{\numYearTwoLog}{39+}
\newcommand{\numYearTwoSurvey}{23}

%% \newcommand{\pFiveOne}{p5/1}
%% \newcommand{\pFiveTwo}{p5/2}
%% \newcommand{\pFiveOne}{p5/y1}
%% \newcommand{\pFiveTwo}{p5/y2}
\newcommand{\pFiveOne}
%% {\textbf{\color{p5pink}{p5/y1}}}
{\textbf{\color{y1Color}{p5/y1}}}
\newcommand{\pFiveTwo}
%% {\textbf{\color{p5pink}{p5/y2}}}
{\textbf{\color{y2Color}{p5/y2}}}
%% \newcommand{\pFiveOne}{\textsc{p5-1}}
%% \newcommand{\pFiveTwo}{\textsc{p5-2}}
%% \newcommand{\pFiveOne}{\ensuremath{\mathsf{p5/1}}}
%% \newcommand{\pFiveTwo}{\ensuremath{\mathsf{p5/2}}}

%% participants
%% \newcommand{\yOneP}[1]
%%   {{\color{y1Color}{\textbf{P0}}}}
%% \newcommand{\yTwoP}[1]
%%   {{\color{y2Color}{\textbf{P0}}}}
\newcommand{\pA}[1]
{{\color{y1Color}{\textbf{A#1}}}}
\newcommand{\pB}[1]
{{\color{y1Color}{\textbf{B#1}}}}
\newcommand{\pC}[1]
{{\color{y2Color}{\textbf{C#1}}}}
\newcommand{\pD}[1]
{{\color{y2Color}{\textbf{D#1}}}}

\newcommand{\pQuote}[1]
{\textit{``#1''}}


%% \def\sectionautorefname{\S\!}
%% \def\subsectionautorefname{\S\!}
%% \def\subsubsectionautorefname{\S\!}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% \def\parahead#1
%%   %% {\paragraph{\textbf{#1.}}}
%%   {\paragraph{\textit{#1.}}}

\newcommand{\parahead}[1]
{%
  \vspace{0.07in}%
  \noindent%
  \textbf{\textit{#1.}}%
}

% \def\subsubsec#1
%   {\subsubsection*{\textit{#1}}}

\def\subsubsec#1
{\subsubsection{#1}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\inlineFig}[1]{%
  \begingroup\normalfont
  % \vspace*{-0.1cm}
  \includegraphics[height=1.2\fontcharht\font`\B]{#1}%
  \endgroup
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \newcommand{\takeaway}[1]
% {\textbf{T#1}}

% \newcommand{\takeawayStatic}
% {\takeaway{1}}

% \newcommand{\takeawayLive}
% {\takeaway{2}}

% \newcommand{\takeawayClutter}
% {\takeaway{3}}

% \newcommand{\takeawaySkeptic}
% {\takeaway{4}}


\newcommand{\takeaway}[1]
{  \begingroup\normalfont
  % \vspace*{-0.1cm}
  \includegraphics[height=1.3\fontcharht\font`\B]{#1}%
  \endgroup}

\newcommand{\takeawayStatic}
{\takeaway{pictures/t1.pdf}}

\newcommand{\takeawayLive}
{\takeaway{pictures/t2.pdf}}

\newcommand{\takeawayClutter}
{\takeaway{pictures/t3.pdf}}

\newcommand{\takeawaySkeptic}
{\takeaway{pictures/t4.pdf}}


\newcommand{\takeawayGeneric}
{\takeaway{pictures/tx.pdf}}



\setuldepth{Berlin}
\definecolor{linkColor}{HTML}{257E98}
\newcommand\asLink[2]{\textcolor{linkColor}{\href{#1}{\ul{#2}}}}


%%%%%%%%%%%%%%%%%

